Approximately optimal domain adaptation with Fisher's Linear Discriminant

We propose a class of models based on Fisher's Linear Discriminant (FLD) in the context of domain adaptation. The class is the convex combination of two hypotheses: i) an average hypothesis representing previously seen source tasks and ii) a hypothesis trained on a new target task. For a particular generative setting we derive the optimal convex combination of the two models under 0-1 loss, propose a computable approximation, and study the effect of various parameter settings on the relative risks between the optimal hypothesis, hypothesis i), and hypothesis ii). We demonstrate the effectiveness of the proposed optimal classifier in the context of EEG- and ECG-based classification settings and argue that the optimal classifier can be computed without access to direct information from any of the individual source tasks. We conclude by discussing further applications, limitations, and possible future directions.

==> iclr2021/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/02_pami_introduction.tex <==
\section{Introduction}

\IEEEPARstart{F}{or}  problems with limited context-specific labeled data, machine learning models often fail to generalize well. Modern machine learning approaches such as transfer learning~\citep{pan2010survey, weiss2016survey}, domain adaptation~\citep{ sun2015survey}, meta-learning~\citep{vilalta2002perspective,  vanschoren2019meta,finn2019online, hospedales2021meta}, and continual learning~\citep{van2019three, hadsell2020embracing,de2021continual,  vogelstein2022representation} can mitigate this ``small data effect" but still require a sufficient amount of context-specific data to train a model that can then be updated to the context of interest. These approaches are either ineffective or unavailable for problems where the input signals are highly variable across contexts or where a single model does not have access to a sufficient amount of data due to privacy or resource constraints \citep{muhlhoff2021predictive}. Note that the terms ``context'' and ``task'' can be used interchangeably here. In this paper we deal with the physiological predictive problem -- a problem with both high variability across contexts (e.g., different recording sessions or different people) and privacy constraints (e.g., biometric data is often considered sensitive and identifiable and should not be shared freely across devices).

We define the physiological predictive problem as any setting that uses biometric or physiological data (e.g., EEG, ECG, breathing rate, etc.) or any derivative thereof to make predictions related to the state of a person. The predicted state could be as high level as the person's cognitive load or affect \citep{10.3389/fnhum.2019.00191} or as low level as which hand they are trying to move \citep{10.3389/fnins.2018.00130}. The machine learning models for these problems often use expert-crafted features and a relatively simple model such as a polynomial classifier or regressor \citep{eeg-da}.

The standard cognitive load classification baseline using EEG data, for example, is a linear model trained using the band powers of neuroscientifically relevant frequencies (e.g., the theta band from 4-7 Hz, the alpha band from 8-12 Hz, etc. \citep{kandel2021principles}) as features \citep{akrami2006eeg, 8741944, GUERRERO2021e07258}. Recent systems for mental state classification have explored more complicated feature sets \citep{10.3389/fnhum.2022.930291} to the tune of some success. Similarly, popular ECG-based predictive systems use simple statistics related to the inter-peak intervals as features for a linear classifier to predict cognitive state \citep{mcduff2014remote, lee2022mental}. Outperforming these simple systems is more challenging for physiological prediction compared to domains such as computer vision and natural language processing because of the high variability and privacy limitations of the input data.

To be more specific, a common approach used in modern machine learning methods is to leverage data from multiple tasks to learn a representation of the data that is effective for every task~\citep{baxter2000model,zhang2018overview}. Once the representation is learned from the set of tasks it can then be applied to a new task and it is assumed that the representation is similarly effective for it. If the variability across the different tasks is high then data from a large set of tasks is necessary to learn a generalizable representation~\citep{baxter2000model}. For physiological predictive systems, there is context variability caused by changes in sensor location or quality, changes in user, and changes in environmental conditions. Hence, the variability across physiological predictive contexts is high and data from a large set of contexts is necessary to learn a transferable representation. Unfortunately, collecting data from a large set of relevant physiological contexts can be prohibitively expensive.

% Further complicating the use of standard modern machine learning methods for physiological predictive problems is that users of a device or participants in a study will often not want their biometric data to be shared or pooled in any way. Methods that do not require a centralized data pool, then, are required. [needs more content? is this privacy part even necessary?]

In this paper we propose a class of models based on Fisher's Linear Discriminant (``FLD")~\citep{izenman2013linear, devroye2013probabilistic} that interpolates between i) a model that is a combination of linear models trained on previous source contexts and ii) a linear model trained only on data from a new target context. We study the class of models in a particular generative setting and derive an analytical form of the risk under the 0-1 loss with respect to the target distribution. Using this analytical risk expression, we show that we can obtain an optimal combination of model i) and model ii), that improves generalization on the target context. We compare the performance of the optimal combination to the performance of model i) and model ii) across various generative parameter settings. Finally, we empirically demonstrate that by using the analytical form of the target risk we can improve upon the performance of model i) and model ii) in real-world physiological predictive settings.


==> sections/04_pami_background.tex <==
\section{A Generative Model}
\label{sec:generative-model}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/illustrative-figure/illustrative-figure-tfld-3d-no-axes.PNG}
    \caption{A geometric illustration of the generative assumptions, information constraints, and the model class under study. The red dots represent the data from the target distribution, the red arrow represents an estimate of the projection vector for the target distribution, the grey arrows represent source projection vectors, the blue arrow represents the average-source projection vector, and the green line interpolating between the blue and red arrows represents the possible end points of a convex combination of the red and blue arrows.}
    \label{fig:illustrative-figure}
\end{figure*}

Our goal is to develop a private (in some sense, see Section\ref{subsec:privacy}) and optimal classifier that can leverage information from data drawn from the target and source distributions. For this purpose, we first put relatively strict generative assumptions on the data and then make the relationship between the target distribution and the source distributions explicit.

In particular, we assume that $ \mc{P}^{(j)} $ is a binary classification distribution that can be described as follows:
\begin{align}
\label{eq:model-assumptions}
    \scalemath{0.90}{
    \mc{P}^{(j)} = \pi^{(j)} \;\mathcal{N}\left(\nu^{(j)}, \Sigma^{(j)}\right) + (1 - \pi^{(j)}) \;\mathcal{N}\left((-1)\nu^{(j)}, \Sigma^{(j)}\right)}
\end{align} for $j \in \{0, \hdots, J\}$.That is, $ \mc{P}^{(j)} $ is a mixture of two Gaussians such that the midpoint of the class conditional means is the origin and that the class conditional covariance structures are equivalent. Note that $\mc{P}^{(j)}$ is uniquely parameterized by $\nu^{(j)}, \Sigma^{(j)},$ and $\pi^{(j)}$. It is known that Fisher's Linear Discriminant function is optimal under 0-1 loss for distributions of the form described in Eq. \eqref{eq:model-assumptions}~\citep[Chapter~4]{devroye2013probabilistic}. Recall that Fisher's Linear Discriminant function is the classifier defined as
\begin{align}
\label{eq:fld}
    h_{FLD}(x) = \mathbb{1}\left\{\omega^{\top} x > c\right\},
\end{align} where $ \mathbb{1}\{s\} $ is 1 if $ s $ is true and $ 0 $ otherwise and where
\begin{align*}
    \scalemath{0.95}{
    \omega = (\Sigma_0 + \Sigma_1)^{-1} (\nu_1 - \nu_0) \; \; \text{and} \; \; c = \omega^\top \left(\nu_0 + \nu_1\right) + \log \frac{\pi_0}{\pi_1}. }
\end{align*} 
Here $\nu_i, \Sigma_i$ and $\pi_i$ are the mean, covariance matrix, and prior probability pertaining to class $i \in \{0, 1\}$. For a distribution $\mc{P}$ of the form described in Eq. \ref{eq:model-assumptions}, and assuming $ \pi = 0.5 $ for simplicity, the above expressions reduce to $\omega = \frac{1}{2}\Sigma^{-1} (\nu_1 - \nu_0)$ and $c = 0$. From the form of Eq. \eqref{eq:fld} it is clear that the projection vector $\omega$ is a sufficient statistic for classification under 0-1 loss with respect to the distribution $ \mc{P}$. To this end, \textbf{we will assume that for the source distributions we only have access projection vectors $\omega^{(1)}, \hdots, \omega^{(J)}$}. 

We next make a generative assumption about the source projection vectors $\omega^{(1)}, 
\hdots, \omega^{(J)} $ to make the relationship between the distributions explicit. Recall that the von Mises-Fisher (vMF) distribution \citep{fisher1993statistical}, denoted by $\mc{V}(\mu, \kappa)$, has realizations on the $ d $-sphere and is completely characterized by a mean direction vector $ \mu \in \mathbb{R}^{d} $ and a concentration parameter $ \kappa \in \mathbb{R}_{\ge 0} $. When the concentration parameter is close to $ 0 $ the vMF distribution is close to a uniform distribution on the $ d$-sphere. When the concentration parameter is large, the vMF distribution resembles a normal distribution with mean $ \mu $ and a scaled isotropic variance proportional to the inverse of $ \kappa $. 

For our analysis we assume that the source vectors $ \omega^{(1)}, \hdots, \omega^{(J)}  \stackrel{iid}{\sim} \mathcal{V}(\mu, \kappa) $ for unspecified $ \mu $ and $ \kappa $. This assumption forces additional constraints on the relationship between $ \nu^{(j)} $ and $ \Sigma^{(j)} $ in the context of Eq. \eqref{eq:model-assumptions} -- namely that $ || (\Sigma^{(j)})^{-1}\nu^{(j)} ||_{2} = \sqrt{2} $. In our simulated settings below, the generative models adhere to this constraint. In practical applications, we can use the (little) training data that we have access to force our estimates of $ \nu $ and $ \Sigma $ to be conformant. 

\subsection{A Simple Class of Classifiers}

With the generative assumptions described above, we propose a class of classifiers $ \mc{H} $ that can effectively leverage the information available with just access to the projection vectors:
\begin{align*}
     \scalemath{0.8}{
     \mc{H} := \Bigg\{ \quad h_{\alpha}(x) = \mathbb{1} \left\{  \left( \underbrace{\alpha \omega^{(0)} + (1 - \alpha) \sum_{j=1}^{J} \omega^{(j)}}_{\omega_{\alpha}}\right)^{\top}x > 0\right\} : \alpha \in [0,1] \Bigg\}}
    % &\mc{H} := \Bigg\{ \\ & \quad h_{\alpha}(x) = \mathbb{1} \left\{  \left( \underbrace{\alpha \omega^{(0)} + (1 - \alpha) \sum_{j=1}^{J}
    % \omega^{(j)}}_{\omega_{\alpha}}\right)^{\top}x > 0\right\} \\&\hspace{6.5cm}: \alpha \in [0,1] \Bigg\}.
\end{align*} The set $ \mc{H} $ is exactly the classifiers parameterized by the convex combinations of the target projection vector and the sum of the source projection vectors. We refer to this convex combination as $ \omega_{\alpha} $.  Letting $ \bar{\omega} := \frac{1}{J}\sum_{j=1}^{J} \omega^{(j)} $, we note that $ \omega_{\alpha} $ can be reparametrized in the context of the vMF distribution with the observation that
\begin{align*}
    (1-\alpha) \sum_{j=1}^{J} \omega^{(j)} &= \frac{J(1 - \alpha)||\bar{\omega}||}{||\bar{\omega}||} \bar{\omega} \\
    &= J(1-\alpha)||\bar{\omega}|| \; \hat{\mu},
\end{align*} where $ \hat{\mu} = \bar{\omega} / ||\bar{\omega} || $ is the maximum likelihood estimate for the mean direction vector of the vMF distribution. By letting $ \alpha \gets \frac{\alpha}{\alpha + J (1-\alpha)||\bar{\omega}||}$ 
% and appropriately scaling $ c_{\alpha} $ 
we maintain the same set $ \mc{H} $ but make the individual classifiers more amenable to analysis. Figure \ref{fig:illustrative-figure} illustrates the geometry of $ \mc{H} $ for $ d = 3 $.

We view different decision rules in $ \mc{H} $ as elements along a classical bias-variance trade off curve parameterized by $ \alpha $ \citep{belkin2019reconciling}. In particular, when the amount of data available from the target distribution is small, the projection induced by an $ \alpha $ value closer to 1 can be interpreted as a high variance, low bias estimate of the target projection vector. Conversely, an $ \alpha $ value of 0 can be interpreted as a low variance, high bias estimate. In situations where the concentration parameter $ \kappa $ is relatively large, for example, we expect to prefer combinations that favor the average-source vector. We discuss this in more detail and in the context of different parameter settings for our generative model in Section \ref{subsec:simulations}.

\subsection{Approximating optimality}\label{subsec:approximating-optimality} 


% Using properties of the normal and vMF distributions for  ``large" $ J $, we have,
% \begin{align*}
%     \hat{\omega}^{(0)} \sim \mathcal{N}\left(\omega^{(0)}, \frac{1}{4n \pi(1-\pi)} \Sigma^{(0)}\right) \quad \quad \text{ and} \quad \quad \hat{\mu} \sim \mathcal{N}\left(\mu, \Psi \right),
% \end{align*} where $\Psi$ is the squared standard error of the estimate $\hat \mu$ [either cite or define in the text]. 
% Thus letting $ \hat{\omega}_{\alpha} = \alpha \hat{\omega}^{(0)} + (1-\alpha) \hat{\mu} $ and using independence, we have
% \begin{equation*}
% \label{dist-properties}
% \hat{\omega}_{\alpha} \sim \mathcal{N}\left(\alpha \omega^{(0)} + (1-\alpha) \mu,  \frac{\alpha^{2}}{4n \pi(1-\pi)} \Sigma^{(0)} + (1-\alpha)^{2} \Psi\right)
% \end{equation*} for ``large" $ J $.

We define the optimal classifier $ h_{\alpha^{*}} $ in the set $ \mc{H} $ as the classifier that minimizes the expected risk with respect to the target distribution $ \mc{P}^{(0)} $. Given the projection vectors  $ \{\omega^{(j)}\}_{j=1}^{J} $ and the target class conditional mean and covariance, $ \nu^{(0)} $ and $ \Sigma^{(0)} $, the risk (under the 0-1 loss) of a classifier $ h_{\alpha} \in \mc{H} $ is
\begin{equation*}
\label{risk}
    R \left( h_{\alpha} \mid \{\omega^{(j)}\}_{j=1}^{J}, \nu^{(0)}, \Sigma^{(0)} \right) = \Phi \left( \frac{-\omega_{\alpha}^\top \nu^{(0)}}{\sqrt{\omega_{\alpha}^\top \Sigma^{(0)} \omega_{\alpha}}} \right)
    % \ell (h_{\alpha}| \{(\omega^{(j)}, c^{(j)})\}_{j=1}^{J}, \nu^{(0)}, \Sigma^{(0)}) = \pi  \Phi \bigg( \frac{-\omega_{\alpha}^\top \nu^{(0)} + c_{\alpha}}{\sqrt{\omega_{\alpha}^\top \Sigma^{(0)} \omega_{\alpha}}} \bigg) + (1-\pi) \Phi \bigg( \frac{-\omega_{\alpha}^\top \nu^{(0)} - c_{\alpha}}{\sqrt{\omega_{\alpha}^\top \Sigma^{(0)} \omega_{\alpha}}} \bigg)
\end{equation*} 
for $\mathcal{P}^{(0)} $ of the form described in Eq. \eqref{eq:model-assumptions} and where $ \Phi $ is the cumulative distribution function of the standard normal. The derivation is given in the \cref{sec:app-derivation}. In practice, the source projection vectors, source thresholds, target class conditional mean and covariance structure are all estimated. Based on the above risk, we can define the expected risk of $h_{\alpha}$ as,
\begin{equation}
\label{eq:risk-integral}
    \mathcal{E}(h_{\alpha}) = \mbb{E}_{\omega_{\alpha}}  \left[ R \left(h_{\alpha} \mid \{\omega^{(j)}, \}_{j=1}^{J}, \nu^{(0)}, \Sigma^{(0)}\right)\right].
\end{equation}
Unfortunately, despite the strong distributional assumptions we have in place, the expected risk is too complicated to analyze entirely.
Instead, we approximate $ \mathcal{E}(h_{\alpha}) $ with $\hat{\mathcal{E}}(h_{\alpha})$, which we can evaluate via Monte Carlo integration by sampling from the distribution of $ \omega_{\alpha} $ (derived in Section \ref{subsec:distribution-of-omega-alpha}) and using the plug-in estimates for $ \nu^{(0)} $ and $ \Sigma^{(0)} $. 

% We can further simplify this expression by assuming $\pi = 1/2$ (equal prior probabilities) and $c_{\alpha} = 0$ (the combined decision rule passes through the origin):
% \begin{equation}
% \label{eq:risk-integral}
%     \mc{E} \approx \hat{\mc{E}} := \mbb{E}_{\omega_{\alpha} \sim \mathcal{N}(\mu_{\omega_{\alpha}}, \Sigma_{\omega_{\alpha}})} \bigg[ \Phi \bigg( - \frac{\omega_{\alpha}^\top \nu^{(0)}}{\sqrt{\omega_{\alpha}^\top \Sigma^{(0)} \omega_{\alpha}}} \bigg) \bigg].
% \end{equation}

% \begin{equation*}
%     \mc{E} \approx \hat{\mc{E}} := \mbb{E}_{\omega_{\alpha} \sim \mathcal{N}(\mu_{\omega_{\alpha}}, \Sigma_{\omega_{\alpha}})} \bigg[ \pi \Phi \bigg( \frac{-\omega_{\alpha}^\top \nu^{(0)} + c_{\alpha}}{\sqrt{\omega_{\alpha}^\top \Sigma^{(0)} \omega_{\alpha}}} \bigg) +  (1-\pi) \Phi \bigg( \frac{-\omega_{\alpha}^\top \nu^{(0)} - c_{\alpha}}{\sqrt{\omega_{\alpha}^\top \Sigma^{(0)} \omega_{\alpha}}} \bigg) \bigg],
% \end{equation*} 

Using this risk function, we can search for optimal $\alpha^\ast$ that minimizes the expected risk over $\alpha \in [0, 1]$. The procedure for calculating $\alpha^\ast$ is outlined in Algorithm \ref{alg:cap}. For the remainder of this section, we use $ \hat{t} $ to denote an estimate of the parameter $ t $.

\begin{algorithm*}[t]
\caption{Calculating the optimal convex coefficient}\label{alg:cap}
\label{alg:optimal}
\begin{algorithmic}[1]
\Require target task class conditional mean $\hat \nu_0^{(0)}$ and $\hat \nu_1^{(0)} $, target task class conditional covariance $\hat \Sigma^{(0)} $, normalized source proj. vectors $\{ \hat \omega^{(j)} \}_{j=1}^J$, the number of bootstrap samples $ B $.
\State
$ \hat \omega^{(0)} \gets \textproc{Normalize} \left( \frac{1}{2} (\hat \Sigma^{(0)})^{-1} (\hat \nu_1^{(0)} - \hat \nu_0^{(0)}) \right)$
\Comment{Estimate the target proj. vector}
\State
$ \hat{\mu} \gets$ \textproc{Normalize}$\left(\frac{1}{J} \sum_{j=1}^{J} \hat \omega^{(j)} \right)$
\Comment{Estimate vMF mean direction vector}
\State
$ \hat \Psi \gets $ \textproc{Variance}$\left(\hat{\mu}\right) $
\Comment{Variance of vMF mean direction vector}
\State
$ \hat \Sigma_{\omega} \gets $ \textproc{Variance}$\left(\hat \omega^{(0)} \right) $ \Comment{Variance of the target proj. vector (see \cref{subsec:distribution-of-omega-alpha})}
\For{each $\alpha \in [0, 1]$}
    \State
    $ \hat \omega_{\alpha} \gets \left(\alpha \; \hat \omega^{(0)} + (1-\alpha)\; \hat{\mu} \right)$ \Comment{Average convex combination}
    \State
    $ \hat \Sigma_{\alpha} \gets \alpha^{2} \hat \Sigma_{\omega} + (1-\alpha)^{2}\hat \Psi $
    \Comment{Variance of average convex combination}
    \For{each $ b $ in $\{1, .. , B\} $}
        \State
        $ \omega_{b} \gets \mc{N}\left(\hat \omega_{\alpha}, \hat \Sigma_{\alpha}\right)$
        \Comment{Sample from appropriate normal distribution}
        \State
        $r_{b} \gets \Phi \left( - \frac{\omega_{b}^{\top} \hat \nu^{(0)}}{\sqrt{\omega_{b}^{\top} \hat \Sigma^{(0)} \; \omega_{b}}} \right) $ \Comment{Calculate error for sample}
    \EndFor
    \State $\hat{\mathcal{E}}\left({\alpha}\right) \gets \frac{1}{B} \sum_{b=1}^{B} r_{b} $ \Comment{Calculate risk}
\EndFor
\State $\alpha^{*} \gets \argmin_{\alpha} \hat{\mathcal{E}} (\alpha)$ \Comment{Select optimal alpha}
\end{algorithmic}
\end{algorithm*}

\subsection{Deriving the asymptotic distribution of $ \hat{\omega}_{\alpha} $}
\label{subsec:distribution-of-omega-alpha}

We are interested in deriving a data-driven method for finding the element of $ \mc{H} $ that performs best on the target task. For this, we rely on the asymptotic distribution of $ \hat{\omega}_{\alpha} = \alpha \hat{\omega}^{(0)} + (1-\alpha) \hat{\mu} $. 
% To keep the notations clear, we will refer to the parameters $t^{(0)}$ associated with target distribution as simply $t$. 
First, we consider the estimated target projection vector $\hat \omega^{(0)} = \frac{1}{2} (\hat \Sigma^{(0)})^{-1} (\hat\nu_1^{(0)} - \hat\nu_0^{(0)})$ as a product of the independent random variables, $A := n (\hat \Sigma^{(0)})^{-1}$ and $\tau := \frac{1}{2}(\hat\nu_1^{(0)} - \hat\nu_0^{(0)})$ and note that $A \sim W_{d}(n, \Sigma^{(0)})$ is distributed according to a Wishart distribution with $n$ degrees of freedom and scatter matrix $\Sigma^{(0)}$ and that $\tau \sim \mc{N}_d(\nu^{(0)}, \Sigma^{(0)} / n)$ is normally distributed. 
For large $n$, the random vector $nA^{-1}\tau$ has the asymptotic distribution given by,
\[ 
\sqrt{n} \left( nA^{-1}\tau - (\Sigma^{(0)})^{-1} \nu \right) \stackrel{d}{\longrightarrow} \mc{N}_d(0, \tilde{\Sigma}),
\]
where $\tilde{\Sigma} = (1 + (\nu^{(0)})^\top (\Sigma^{(0)})^{-1} \nu^{(0)}) (\Sigma^{(0)})^{-1} - (\Sigma^{(0)})^{-1} \nu^{(0)} (\nu^{(0)})^\top (\Sigma^{(0)})^{-1} $ \citep{kotsiuba2016asymptotic}. It follows that $\hat \omega^{(0)}$ is aymptotically distributed according to a normal distribution with mean $\omega^{(0)} = (\Sigma^{(0)})^{-1} \nu^{(0)}$ and covariance matrix $\Sigma_{\omega} := \tilde{\Sigma} / n$. 

Next, we observe that $\hat \mu$ is the sample mean direction computed from $J$ i.i.d samples drawn from a $\mathcal{V}(\mu, \kappa)$. For large $J$ we have $\hat \mu$ asymptotically distributed as a normal distribution with mean $\mu$ and covariance $\Psi$ given by 
\[
\Psi = \left( \frac{1 - \frac{1}{J} \sum_{j=1}^{J} (\mu^\top \omega^{(j)})^2}{J \| \bar\omega \|} \right)^{1/2} I_d,
\]
where $I_d$ is the $d \times d$ identity matrix \citep{fisher1993statistical}. 

Finally, since $\hat \omega$ and $\hat \mu$ are independent and asymptotically normally distributed, for large $n$ and $J$, we have that
\begin{equation}
\label{risk-integral}
\hat{\omega}_{\alpha} \sim \mathcal{N}\left(\underbrace{\alpha \omega^{(0)} + (1-\alpha) \mu}_{\omega_{\alpha}}, \underbrace{\alpha^2 \Sigma_{\omega} + (1-\alpha)^{2} \Psi}_{\Sigma_{\alpha}}\right).
\end{equation}

We use samples from this asymptotic distribution when evaluating the risk function described in Eq. \eqref{eq:risk-integral}. 

==> sections/bivariate_two_task_case.tex <==
\section{Fisher's Linear Discriminant}

The decision rule of the Fisher's Linear Discriminant (FLD) for a binary classification problem is given by,
\begin{equation}
   h(x; \omega, c) = 
    \begin{cases}
        1 & \omega^\top x > c \\
        0 & \text{otherwise}
    \end{cases}
\end{equation}
where, 
\begin{align}
    \omega &= (\hat \Sigma_0 + \hat \Sigma_1)^{-1} (\hat \mu_1 - \hat \mu_0) \notag \\
    c &= \omega^\top \bigg( \frac{\hat \mu_1 + \hat \mu_0}{2} \bigg) + 2 \log \frac{1-\hat \pi}{\hat \pi} \notag
\end{align}
In the above expressions, $\hat \mu_k$ and $\hat \Sigma_k$ are the sample mean and covariance matrix of class $k$ ($k \in \{0, 1\}$) and $\hat \pi$ is the sample proportion (prior probability) of class 1.

\section{Analysis when $d>2$, $J>1$}

We have $n$ samples from a target task, denoted by $\Dt = \{ (x_i, y_i) \}_{i=1}^n \sim \Pt$ and $m$ samples from a source task denoted by $\Ds^j = \{ (x_i^j, y_i^j)\}_{i=1}^m \sim \Ps^j$, where $x \in X \subseteq \mathbb{R}^d$, $y \in Y = \{ 0, 1 \}$, and $j \in \{ 1, \dots, J\}$. The target task distribution $\Pt$ is characterized by the class conditional densities,
\begin{equation}
    f_{k,t} \stackrel{d}{=} \mathcal{N}((-1)^{k+1}\mu, I_d), \notag
\end{equation}
while the source task distribution $\Ps^j$ is characterized by the class conditional densities,
\begin{equation}
    f_{k,s^j} \stackrel{d}{=} \mathcal{N}((-1)^{k+1}R(\nu_j) \mu, I_d). \notag
\end{equation}
Here, $k \in \{0, 1\}$, $\mu = [ 1, 0_{d-1}]^\top$ and $R(\nu)$ is a rotational matrix given by, 
\begin{equation}
    R(\nu) = 2 \frac{(\mu + \nu)(\mu + \nu)^\top}{(\mu + \nu)^\top(\mu + \nu)} - I_d \notag
\end{equation}
where, $\nu \sim \text{VMF}(\mu, \kappa)$ is sampled from the Von Mises-Fisher distribution. All the target and source tasks have the same label distribution, i.e. $p(y_t=1) = p(y_{s^j}=1) = \pi$.

Let $h_t(x; \omega_t, c_t)$ be a FLD decision rule trained with target task data $\Dt$ and $h_{s^j}(x; \omega_{s^j}, c_{s^j})$ be a FLD decision rule trained with $j$-th source task data $\Ds^j$. We consider a classifier $g_{\alpha}(x)$ defined as, 
\begin{equation}
    g_\alpha(x) = 
    \begin{cases}
        1 & \omega_{\alpha}^\top x > c_{\alpha} \\
        0 & \text{otherwise}
    \end{cases}
\end{equation}
where, 
\begin{align}
     \omega_{\alpha} &= \alpha \omega_t + (1-\alpha) \sum_{j=1}^J \omega_{s^j} \notag \\
     c_{\alpha} &= \alpha c_t + (1-\alpha) \sum_{j=1}^J c_{s^j} \notag
\end{align}

We make several assumptions to simplify our analysis: (1) The sample class covariance matrices are known and are equal to the identity matrix ($\hat \Sigma_0 = \hat \Sigma_1 = I_d$), (2) bisector of sample class means is equal to zero ($\frac{\hat \mu_0 + \hat \mu_1}{2} = 0$), and (3) sample class proportion is equal to the true class proportion ($\hat \pi = \pi$). Under these assumptions $\omega_t$ and $c_t$ can be written as, 
\begin{align}
    \omega_t &= \frac{\hat \mu_1 - \hat \mu_0}{2}, \notag \\
    c_t &= 2 \log \frac{1-\pi}{ \pi}. \notag
\end{align}
Since the class conditional densities are normal, we have $\hat \mu_1 \sim \mathcal{N}(\mu, \frac{I_d}{n\pi})$ and $\hat \mu_0 \sim \mathcal{N}(-\mu, \frac{I_d}{n(1-\pi)})$. Therefore, $\omega_t$ is also normally distributed with $\omega_t \sim \mathcal{N}(\mu, \frac{I_d}{4n \pi(1-\pi)})$. Similarly, we can show that the projection term $\omega_{s^j}$ of the $j$-th source task has the conditional distribution $\omega_{s^j} \mid \nu_j \sim \mathcal{N}(R(\nu_j)\mu, \frac{I_d}{4m \pi(1-\pi)})$, while the threshold term $c_{s^j}$ is equal to 2 $\log \frac{1-\pi}{ \pi}$. Building off these intermediate results, we can find the conditional expected value $\mu_{\omega_{\alpha}}$ and variance $\Sigma_{\omega_{\alpha}}$ of the combined projection term $\omega_{\alpha}$, given $\{ \nu_j \}_{j=1}^J$:
\begin{align}
    \mu_{\omega_{\alpha}} = \mathbb{E}[\omega_{\alpha} \mid \{ \nu_j \}_{j=1}^J] &= \alpha \mathbb{E}[\omega_t] + (1-\alpha) \sum_{j=1}^J \mathbb{E}[\omega_{s^j} \mid \{ \nu_j \}_{j=1}^J] \notag \\
    &= \alpha \mu + (1-\alpha) \sum_{j=1}^J R(\nu_j) \mu  \notag \\
    &= \bigg( \alpha I_d + (1-\alpha) \sum_{j=1}^J R(\nu_j) \bigg) \mu  \notag, \\
    \Sigma_{\omega_{\alpha}} = \Var[\omega_{\alpha} \mid \{ \nu_j \}_{j=1}^J] &= \alpha^2 \Var[\omega_t] + (1-\alpha)^2 \sum_{j=1}^J \Var[\omega_{s^j} \mid \{ \nu_j \}_{j=1}^J] \notag \\
    &= \alpha^2 \frac{I_d}{4n \pi(1-\pi)} + (1-\alpha)^2 \sum_{j=1}^J \frac{I_d}{4m \pi(1-\pi)} \notag \\
    &= \frac{1}{4\pi (1-\pi)} \bigg( \frac{\alpha^2}{n} + \frac{(1-\alpha)^2 J}{m} \bigg) I_d \notag.
\end{align}
Since $\omega_{\alpha}$ is a weighted sum of normal random variables, we can conclude that $\omega_{\alpha} \mid \{ \nu_j \}_{j=1}^J \sim \mathcal{N}(\mu_{\omega_{\alpha}},  \Sigma_{\omega_{\alpha}})$. Furthermore, we can find an expression for $c_{\alpha}$ as follows:
\begin{align}
    c_{\alpha} &= \alpha c_t + (1-\alpha) \sum_{j=1}^J c_{s^j} \notag \\
    &= 2 \alpha \log \frac{1-\pi}{ \pi} + 2 (1-\alpha) \sum_{j=1}^J \log \frac{1-\pi}{ \pi} \notag \\
    &= 2(\alpha + (1-\alpha)J) \log \frac{1-\pi}{ \pi} \notag.
\end{align}
The generalization error on the target task of the classifier $g_{\alpha}(x)$ is given by,
\begin{align}
    p(g_{\alpha}(x) \neq y \mid x, \omega_{\alpha}, \{ \nu_j \}_{j=1}^J) &= \frac{1}{2} p_{x \sim f_{1,t}}[\omega_{\alpha}^\top x < c_{\alpha}] + \frac{1}{2}p_{x \sim f_{0, t}}[\omega_{\alpha}^\top x > c_{\alpha}] \notag \\
    &= \frac{1}{2} +  \frac{1}{2} p_{x \sim f_{1,t}}[\omega_{\alpha}^\top x < c_{\alpha}] - \frac{1}{2}p_{x \sim f_{0, t}}[\omega_{\alpha}^\top x < c_{\alpha}] \notag \\
    &= \frac{1}{2} \bigg[ \Phi \bigg( \frac{-\omega_{\alpha}^\top \mu + c_{\alpha}}{\| \omega_{\alpha} \|} \bigg) + \Phi \bigg( \frac{-\omega_{\alpha}^\top \mu - c_{\alpha}}{\| \omega_{\alpha} \|} \bigg) \bigg] \notag.
\end{align}
Let $e_t(g_{\alpha}) = \mathbb{E}_{\{ \nu_j \}_{j=1}^J \sim \text{VMF}(\mu, \kappa)} \big[ \mathbb{E}_{\omega_{\alpha} \sim \mathcal{N}(\mu_{\omega_{\alpha}},  \Sigma_{\omega_{\alpha}})} [ p(g_{\alpha}(x) \neq y \mid x, \omega_{\alpha}, \{ \nu_j \}_{j=1}^J) ] \big]$ be the expected target generalization error on the target task. We compute this expected value using MC-integration. Finally, we obtain the expected balanced accuracy on the target task by $1 - e_t(g_{\alpha})$.

\section{Analytical Results}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/effect-of-kappa-analytical.pdf}
    \caption{Performance and optimal $ \alpha $ as a function of $ \kappa $. \textbf{Top:} The expected accuracy for the three classifiers as a function of the concentration parameter of the Von Mises-Fisher distribution $ \kappa $. Each column corresponds to a different amount of data available from the target task, $ m \in \{10, 20, 40\} $, and includes accuracies for the classifiers for various amounts of source tasks, $ J \in \{1, 10, 100\} $. For this figure we fix the dimension $ d = 5 $ and the amount of data from each of the source tasks $ m = 20 $. \textbf{Bottom:} The optimal $ \alpha $ as a function of $ \kappa $ for varying amounts of source tasks. The optimal $ \alpha $ is calculated using Equation ?.}
    % , we plot the expected accuracy (Y-axis) on the target task against the $\kappa$ values (X-axis) corresponding to the source tasks. We fix the target task sample size and dimensionality of the data to be $n=20$ and $d=5$. We consider 9 different combinations of varying number of source tasks ($J = \{ 1, 10, 100 \}$ denoted by solid, dashed, and dotted lines respectively) and source task sample sizes ($m = \{ 10, 20, 40 \}$ illustrated in left, middle, and right columns respectively). We assume that when there are multiple source tasks, each of them possesses the same sample size $m$. We plot the expected accuracy of 3 different classifiers; an FLD trained only on the target data (red), an equally weighted combination of $J$ FLDs trained on each of the source tasks (yellow), and an optimally weighted combination of the target-specific FLD and the sum of source-specific FLDs (green). It can be observed that with the appropriately chosen weight $\alpha^\ast$, the optimal classifier attains the best expected accuracy on the target task. In the \textbf{bottom row}, we plot the optimal $\alpha^\ast$ (Y-axis) against the the $\kappa$ values (X-axis). Note that the optimal $\alpha^\ast$ depends on the $\kappa$, the number of source tasks $J$, and the number of samples $m$ of each source task. Specifically, it can be observed that when $\kappa$ is very small, the optimal classifier rejects the source-trained hypotheses. But as $\kappa$ increases i.e. the source tasks becomes closer to the target task, the optimal classifier incorporates the source trained hypotheses in addition to the target hypothesis resulting in a boost in accuracy.}
    \label{fig:kappa_vs_acc}
\end{figure*}


\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/effect-of-dimension-analytical.pdf}
    \caption{Performance and optimal $ \alpha $ as a function of dimensionality. \textbf{Top:}
    The expected accuracy for the three classifiers as a function of the concentration parameter of the Von Mises-Fisher distribution $ \kappa $. Each column corresponds to a different amount of source data, $ m \in \{10, 20, 40\} $, and includes accuracies for the classifiers for various amounts of source tasks, $ J \in \{1, 10, 100\} $. For this figure we fix the concentration parameter $ \kappa = 100 $ and the amount of data from the target task $ n = 20 $. \textbf{Bottom:} The optimal $ \alpha $ as a function of $ d $ for varying amounts of source tasks. The optimal $ \alpha $ is calculated using Equation ?.
    }
    % \textbf{Top:} illustrates how the expected accuracy (Y-axis) varies with the dimensionality of the data (X-axis). We keep the target sample size $n$ and $\kappa$-value fixed at $n=20$ and $\kappa = 100$. We observe that in all the considered combinations of source sample sizes $m = \{ 10, 20, 40 \}$ and number of source tasks $J = \{ 1, 10, 100 \}$, the optimal classifier with the aptly picked weights $\alpha^\ast$ outperforms the target specific classifier and the equally-weighted combination of the source-specific classifiers. Because the variance of high-dimensional hypotheses is high under low sample sizes, a downward trend can be noticed in the expected accuracy as the dimentionality increases. However, interestingly, when there are more source tasks ($J=100$ for instance) that are closer to the target task, it can be noticed that a high target task accuracy is maintained by the optimal classifier. In the \textbf{bottom row}, we plot the optimal $\alpha^\ast$ (Y-axis) of the optimal classifier against the dimensionality (X-axis).}
    \label{fig:my_label}
\end{figure*}

\begin{figure}
    \centering
    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figures/mental-math/mental_math_bas_and_alphas.pdf}
    \end{subfigure} \\
    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figures/mental-math/mental_math_histograms.pdf}
    \end{subfigure}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

\clearpage
\section{Deviations between Theory and Implementation}

\begin{enumerate}
    \item In the analysis, we define the projection vector of the combined classifier as,
    \begin{equation}
        \omega_{\alpha} &= \alpha \omega_t + (1-\alpha) \sum_{j=1}^J \omega_{s^j} \notag
    \end{equation}
    In the implementation, first the source projection vectors are summed and converted to a unit vector.
    \begin{equation}
        \omega_s = \frac{\sum_{j=1}^J \omega_{s^j}}{\| \sum_{j=1}^J \omega_{s^j} \|} \notag
    \end{equation}
    Then the projection vector is computed as, 
    \begin{equation}
        \omega_{\alpha} &= \frac{\alpha \omega_t + (1-\alpha) \omega_s}{\| \alpha \omega_t + (1-\alpha) \omega_s \|} \notag
    \end{equation}
    
    \item In the analysis, the covariance matrix of the combined projection vector is given by,
    \begin{equation}
        \Sigma_{\omega_{\alpha}} = \frac{1}{4\pi (1-\pi)} \bigg( \frac{\alpha^2}{n} + \frac{(1-\alpha)^2 J}{m} \bigg) I_d \notag
    \end{equation}
    In the implementation, the following covariance matrix is used:
    \begin{equation}
        \Sigma_{\omega_{\alpha}} = \frac{1}{4\pi (1-\pi)} \bigg( \frac{\alpha^2}{n} + \frac{(1-\alpha)^2}{m} \bigg) I_d \notag
    \end{equation}
    This covariance matrix might not be accurate for two reasons: (1) We have to account for the normalization (2) The identity covariance assumption won't hold true in real-data
    
    \item The analysis assumes that, 
        \begin{itemize}
            \item $\mu = [1, 0, \dots, 0]$
            \item Class covariance matrices are $I_d$
            \item Mid-point of the class means is 0.
            \item $\pi = 0.5$
        \end{itemize}
    The implementation is modified such that thee assumptions are held true except for the $\mu$ and $I_d$ assumptions.
\end{enumerate}

$ \frac{\alpha \mu + (1-\alpha) R\left(\frac{v_{1} + v_{2}}{||v_{2} + v_{2}||}\right)\mu}{||\alpha \mu + (1-\alpha) R\left(\frac{v_{1} + v_{2}}{||v_{2} + v_{2}||}\right)\mu||}$

==> sections/notes.tex <==
plug-in estimates with normalization

figure 1 in appendix - non identity covariance, let's keep it determinant be 1 - 2 dimensional problem, rotations parameterized by theta (theta = 0 to pi)
(how does that hard-ness of estimating the covairance structure effect the differnce in the errors of the plug-in estimate version of the algo and the known covairane version of the algo)

figure 2 in appendix - different class conditional covariances, let's keep them determinant 1 

class conditional cov 1 = identity

class conditional cov 2 = [[a, ..., 0], [0, 1/a, ...,], [0,0,1,0,..], ...]]  = diag[a, 1/a, 1, ..., 1] a = [1, 2, 5, 10, 20]

d=10, J=100, kappa=10, n=20
